Data-driven Rollout for Deterministic Optimal Control

We consider deterministic infinite horizon optimal control problems with nonnegative stage costs. We draw inspiration from learning model predictive control scheme designed for continuous dynamics and iterative tasks, and propose a rollout algorithm that relies on sampled data generated by some base policy. The proposed algorithm is based on value and policy iteration ideas, and applies to deterministic problems with arbitrary state and control spaces, and arbitrary dynamics. It admits extensions to problems with trajectory constraints, and a multiagent structure.

==> Data-Driven_Corrections5.tex <==

CORRECTIONS TO CDC PAPER 

Last Corrections, Sept 26, 2021


SECTION 3





*************************
Change: the value J? 0 (x) being finite is a sufficient condition S
for the state x belonging to the maximum reachable set.

to 
the finiteness of the value J? 0 (x) is a sufficient condition
for the state x to belong to the maximum reachable set.   
HOWEVER I don't understand what is the "maximum reachable set" Please clarify or rephrase.
*************************

*************************
I don't understand the statement: "If the goal is to reach a stopping set
Xs, then the way in which the trajectory approaching to or
arriving at Xs is decided by the shape of the cost function,
which is irrelevant to the above analysis. Still, both the cost
function of ?? and its bound J? 0 can be considered as the S
Lyapunov function candidates for such investigation."

Can you try to clarify or eliminate by saying instead that this is an issue that must be addressed separately 

*************************




SECTION 5


*************************
About: "Thus, we envision our algorithm to be applied for solving problems with hybrid systems, logic constraints, trajectory constraints and multiagent structures."

This sentence repeats in part the content of the preceding one. You may consider modifications.

*************************




==> recycle.tex <==
Although being amendable for modifications, for the existing forms of rollout, difficulties may still arise when the state $x$ and control $u$ consists continuous components, the cost function evaluation for base policy $J_{\mu^0}$ requires some substantial computation that cannot be concatenated with the VI steps \eqref{eq:vi_def} and \eqref{eq:vi_policy} described in Section~\ref{sec:introduction}, or the values $J_{\mu^0}$ are available in a subset of $X$. Situations of this type arises when obtaining $\mu^0$ is a challenge itself and can only be stored for some selective states. The interest in this type of settings arises in view of the abundant availability of data, which could be historical trajectories collected and stored independently. In this work, we address such problems and show that as long as the values of $J_{\mu^0}$ are available over a subset that has the property like \eqref{eq:s0_intro}, nearly identical analysis to the existing rollout variants can be carried through and the cost improvement condition remains valid.




The optimal costs are computed and the iteration numbers required for convergence within $\sigma$ are documented. Those initial states are $\{x^i\}_{i=1}^{12}$, whose numerical values are listed in Table~\ref{table:lmpc_ini}. Some of their optimal cost estimates within $\sigma$ error margin, and the iteration numbers required, are listed in Table~\ref{table:lmpc_jstar}. Note that for $x^8$ and $x^{11}$, the lower bound values $J_{\text{low}}$ are slightly bigger than $J_{\Tilde{\mu}^*}$. This is due to that we terminate the sampling trajectory when the states are $0.1\sigma$ close to the origin. So the contribution of the tail trajectory to the cost is missed in computing the upper bound. The sampled data starting from some different initial states, together with the initial feasible trajectory for $x^0$, are shown in Fig.~\ref{fig:lmpc_sample}.   
\begin{table}[h!]
\caption{Initial states used in Example~\ref{eg:lmpc_lqr}}
\label{table:lmpc_ini}
\centering
\begin{tabular}{ |c|c|c|c| } 
\hline
$x^1$ & $x^2$ & $x^3$ & $x^4$ \\
\hline
$[-3\, -0.2]^{\text{T}}$ & $[-2\, -1]^{\text{T}}$ & $[-1\, 0]^{\text{T}}$ & $[1\, 0]^{\text{T}}$ \\
\hline
$x^5$ & $x^6$ & $x^7$ & $x^8$\\
\hline
$[1\, 1]^{\text{T}}$ & $[2\, 1]^{\text{T}}$ & $[1\, -0.5]^{\text{T}}$ & $[2\, -0.5]^{\text{T}}$\\
\hline
$x^9$ & $x^{10}$ & $x^{11}$ & $x^{12}$ \\
\hline
$[3.5\, 0.1]^{\text{T}}$ & $[3.5\, 0.5]^{\text{T}}$ & $[3.6\, 0.3]^{\text{T}}$ & $[-1\, 2]^{\text{T}}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Some initial states, their iteration numbers, the corresponding optimal cost estimates obtained by LMPC, and the lower bounds in Example~\ref{eg:lmpc_lqr}}
\label{table:lmpc_jstar}
\centering
\begin{tabular}{ |c|c|c|c| } 
\hline
$x^i$  & $x^0$ & $x^1$ & $x^5$ \\
\hline
Iteration & $2$ & $1$ & $1$ \\
\hline
$J_{\Tilde{\mu}^*}$ & $49.9164$ & $31.0406$ & $14.7885$ \\
\hline
$J_{\text{low}}$ & $49.9164$ & $31.0411$ & $14.7887$\\
\hline
$x^i$  & $x^8$ & $x^{10}$ & $x^{11}$ \\
\hline
Iteration & $1$ & $1$ & $1$ \\
\hline
$J_{\Tilde{\mu}^*}$ & $8.2034$ & $52.3552$ & $48.2003$ \\
\hline
$J_{\text{low}}$ & $8.2033$ & $52.3552$ & $48.1998$ \\
\hline
\end{tabular}
\end{table}


We will also provide lower bounds $J_{\text{low}}$ of optimal cost $J^*$ in examples~\ref{eg:lmpc_lqr} and \ref{eg:lmpc_hybrid} to indicate the optimality gap. The lower bounds are computed via applying VI algorithm \eqref{eq:vi_def} with $J_0$ set to be the solution of Riccati equation solution for the unconstrained linear-quadratic problem and performing $2$ steps of \eqref{eq:vi_def}, in the case of example~\ref{eg:lmpc_lqr}; and $J_0$ as identically zero, e.g., $J_0\equiv 0$, and performing $10$ steps of \eqref{eq:vi_def}, in the case of example~\ref{eg:lmpc_hybrid}. The reasons due to which those are lower bounds of $J^*$, and the details of the lower bound computation are neglected due to limit of space.

Despite their validity to a broad class of problems, the VI and PI algorithms suffer from the \emph{curse of dimensionality}, which refers to the explosion of the
computation as the cardinality of $X$ increases. One such case is when $X$ is a subset of Euclidean space, where discretization is required in order to perform VI or PI. The difficulty is significantly exacerbated when additional constraints are imposed on entire trajectories of state and control pairs. For a system $z_{k+1}=f_z(z_k,u_k)$ with $z_k\in Z$ and $u_k\in U$, if a set membership constraint of the trajectory is required, e.g., $\{(z_k,u_k)\}\in C_\infty\subset(Z\times U)^\infty$, one needs to introduce an auxiliary state $e_k$ that subsumes all the information of the partial trajectory $\{(z_i,u_i)\}_{i=0}^{k-1}$ relevant to $C_\infty$, and to use as state $x_k=(z_k,e_k)$ and as dynamics $f=(f_z,f_e)$ with mapping $f_e$ defined for $e_k$ accordingly, in order to apply the VI and PI algorithms. When the auxiliary state is defined as $e_k=(z_0,u_0,\dots,z_{k-1},u_{k-1})$, the state space $X$ becomes $Z\cup Z\times \big(\cup_{i=1}^\infty(Z\times U)^i\big)$, which makes the VI and PI unpractical, with even a modest size $Z$.


A direct implication of Prop.~\ref{prop:classic}(a) is that for all stationary policies $\mu$, with $J$ and $J'$ per the statement, we have 
\begin{equation*}
    g\big(x,\mu(x)\big)+J\big(f\big(x,\mu(x)\big)\big)\leq g\big(x,\mu(x)\big)+J'\big(f\big(x,\mu(x)\big)\big).
\end{equation*}
Another immediate consequence is that the inequality \eqref{eq:monotone} preserves when taking infimum over $u\in U(x)$ on both sides. A consequence of Prop.~\ref{prop:classic}(b) is that for all stationary policies $\mu$ we have
\begin{align*}
    &\inf_{u\in U(x)}\big\{g(x,u)+J_\mu\big(f(x,u)\big)\big\}\\
    \leq& g\big(x,\mu(x)\big)+J_\mu\big(f\big(x,\mu(x)\big)\big)=J_\mu(x).
\end{align*}
Then by applying Prop.~\ref{prop:classic}(a) with $J$ as $\inf_{u\in U(x)}\big\{g(x,u)+J_\mu\big(f(x,u)\big)\big\}$, and $J'$ as $J_\mu$, one can obtains the cost improvement property of PI.


In this work, we consider deterministic infinite horizon optimal control problems involving stationary system dynamics
\begin{equation}
\label{eq:dynamics}
    x_{k+1}=f(x_k,u_k),\quad k=0,\,1,\,\dots,
\end{equation}
where $x_k$ and $u_k$ are state and control at stage $k$, and belong to state and control spaces $X$ and $U$, respectively, and $f$ maps $X\times U$ to $X$. The control $u_k$ must be chosen from a nonempty constraint set $U(x_k)\subset U$ that may depend on $x_k$. The cost of $x_k$ and applying $u_k$ is denoted as $g(x_k,u_k)$, which is assumed to be nonnegative and can take the value infinity:
\begin{equation}
\label{eq:cost}
    0\leq g(x_k,u_k)\leq\infty,\quad x_k\in X,\,u_k\in U(x_k).
\end{equation}
The infinity stage cost is used to model state constraint. We investigate feedback policies of the form $\pi=\{\mu_0,\,\mu_1,\,\dots\}$, with each $\mu_k$ being a function mapping $X$ to $U$ and satisfying $\mu_k(x)\in U(x)$ for all $x$. The set of all feedback policies is denoted as $\Pi$. We are particularly interested in policies that are invariant over stages, e.g., $\{\mu,\,\mu,\,\dots\}$, which are called \emph{stationary}. When no confusion arises, with a slight abuse of notation, we also denote $\{\mu,\,\mu,\,\dots\}$ as $\mu$. No restriction is assumed on system dynamics \eqref{eq:dynamics}, stage cost \eqref{eq:cost}, state space $X$, and control space $U$, so the problems addressed here are of great generality. 

For a given policy $\pi=\{\mu_0,\,\mu_1,\,\dots\}$, a function $J_\pi$ that maps $X$ to $[0,\infty]$ can be defined pointwise with its value at $x_0\in X$ as
\begin{equation}
\label{eq:pi_cost_function}
    J_\pi(x_0)= \lim_{k\to\infty}\sum_{i=0}^k g(x_i,\mu_i(x_i)), 
\end{equation}
where $x_{i+1}=f(x_i,\mu_i(x_i))$, $i=0,\,1,\,\dots$. We refer the function $J_\pi$ as the \emph{cost function} of policy $\pi$. For a stationary policy $\mu$, its cost function is denoted as $J_\mu$. The optimal cost function $J^*$ is defined as
\begin{equation}
    J^*(x)=\inf_{\pi\in\Pi}J_\pi(x),\quad x\in X.
\end{equation}
A policy $\pi^*\in\Pi$ is called optimal if it attains the minimum of $J_\pi(x)$ over all $\pi\in \Pi$ for all $x\in X$, e.g.,
\begin{equation*}
    J_{\pi^*}(x)=\inf_{\pi\in\Pi}J_\pi(x)=J^*(x),\quad \forall x\in X.
\end{equation*}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth]{Plots/lmpc_hybrid_1_1.eps}
    \caption{Trajectories of $\mu^0$, rollout policy $\Tilde{\mu}^*$ with $\ell=5$, and MPC policy with horizon $10$ and no final stage cost and constraint, starting from $(1,1)$.}
    \label{fig:lmpc_hybrid_1_1}
\end{figure}




We now provide a \textcolor{Green}{variant of our rollout algorithm} that handles the constraint imposed on entire trajectories. Consider the optimal control problems involving dynamics $z_{k+1}=f_z(z_k,u_k)$ with $z_k\in Z$ and $u_k\in U_z(z_k)\subset U$. The stage cost is $g_z:Z\times U\to[0,\infty]$. Suppose the trajectory constraint $C_\infty$ is \textcolor{Orange}{of the set membership type: a given trajectory $\{(z_k,u_k)\}_{k=0}^\infty$ may or may not belong to $C_\infty$. We introduce an auxiliary state denoted by $e_k$. It belongs to a set $E$ and is assumed to subsume all the information of the trajectory $\{(z_i,u_i)\}_{i=0}^{k-1}$ relevant to $C_\infty$. Its dynamics is denoted by $f_e:Z\times E\times U\to E$.} We use the notation $\{e_k\}\cup \{(z_i,u_i)\}_{i=k}^\infty\in C_\infty$ to indicate the complete trajectory $\{(z_i,u_i)\}_{i=0}^\infty$ fulfills the constraint $C_\infty$, with $\{(z_i,u_i)\}_{i=0}^{k-1}$ subsumed by $e_k$. Then the state for the trajectory unconstrained problem is defined through state $x_k=(z_k,e_k)\in X=Z\times E$, with its dynamics given by $x_{k+1}=f(x_k,u_k)=\big(f_z(z_k,u_k),f_e(z_k,e_k,u_k)\big)$, and control constraint $U(x_k)=U_z(z_k)$. Its stage cost is $g(x_k,u_k)=g_z(z_k,u_k)+\delta_{C_e}(e_k)$, where $C_e$ represents the set of $e_k$ such that there exists a tail trajectory $\{(z_i,u_i)\}_{i=k}^\infty$ that fulfills the trajectory constraint $C_\infty$ when concatenated with $\{(z_i,u_i)\}_{i=0}^{k-1}$ that is represented by $e_k$.

Given a sample set $S^0_z\subset Z$, we assume the invariance property \eqref{eq:s0_main} hold \textcolor{Orange}{under the policy} $\mu_z^0$, which is a policy defined for $z$. Starting from any $z\in S^0_z$, we assume resulting complete trajectory fulfills $C_\infty$. For all $z\in S^0_z$, we denote this resulting complete trajectory as $S^0_z(z)$. Then the set $S^0$ for the trajectory unconstrained problem is given as
\begin{equation*}
    S^0=\big\{(z,e)\,\big|\,z\in S^0_z,\,\{e\}\cup S^0_z(z)\in C_\infty\big\},
\end{equation*}
and the function $\Bar{J}_{S^0}$ is defined as $\Bar{J}_{S^0}\big((z,e)\big)=J_{\mu^0_z}(z)+\delta_{S^0}\big((z,e)\big)$. The problem is thus \textcolor{Orange}{transformed to} the trajectory unconstrained form. Thus the algorithm of the basic form can be applied and Prop.~\ref{prop:rollout_basic} holds.

\begin{exmp}\label{eg:lmpc_lqr}(Sample-based state space exploration) Consider the system dynamics given as $f(x,u)=Ax+Bu$, 
\begin{equation}
\label{eq:lqr_dynamics}
    A = \begin{bmatrix}
        1 & 1\\
        0 & 1\end{bmatrix},\;B=\begin{bmatrix}
        0\\
        1\end{bmatrix}.
\end{equation}
The stage cost is given as $g(x,u)=x^{\text{T}}x+u^2+\delta_C(x)$ with constraint set $C=[-4,4]^2$, $U(x)=U=[-1,1]$. We apply as initial state $x^0=[-3.95\, -0.05]^{\text{T}}$. The lookahead length is $\ell=4$. All of above settings are the same as those given in \cite[Example~A]{rosolia2017learning}. Since our analysis shows that the data collected for $x^0$ can also be used for other initial states, provided that initial solution is feasible. Thus, we repeat the above procedure sequentially with new initial states, using the existing collected data, without providing initial feasible solution, \textcolor{Orange}{as opposed to} $x^0$. Owing to limited spaces, the implementation details are omitted and some sampled states are shown in Fig.~\ref{fig:lmpc_sample}.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth]{Plots/lmpc_sample.eps}
    \caption{Sampled data starting from different initial states. The initial feasible trajectory is labelled with $\Tilde{x}$.}
    \label{fig:lmpc_sample}
\end{figure}

\end{exmp}




The trajectory starting from $(8,-9)$ is illustrated in Fig.~\ref{fig:lmpc_hybrid_8_9}. 



\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth]{Plots/lmpc_hybrid_8_9.eps}
    \caption{Trajectories of $\mu^0$, rollout policy $\Tilde{\mu}$ with $\ell=5$, and MPC policy with horizon $10$ and no final stage cost and constraint, starting from $(8,-9)$.}
    \label{fig:lmpc_hybrid_8_9}
\end{figure}





The new path that is found by the rollout method is highlighted in orange in Fig.~\ref{fig:lmpc_tsp_explore}. It can be seen that this path can not be generated by either $\mu^0$ or $\mu^1$. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.53\linewidth]{Plots/tsp_explore_m.eps}
    \caption{The travelling salesman example with rollout method where new samples ABD, ABDC, ABDCA is added to the sample set $S$. The path highlighted in orange is a new path that is found by rollout, which could not be generated by either $\mu^0$ or $\mu^1$.}
    \label{fig:lmpc_tsp_explore}
\end{figure}
